BLeSS: Bio-inspired Low-level Spatiochromatic Similarity Assisted Image Quality Assessment

This paper proposes a biologically-inspired low-level spatiochromatic-model-based similarity method (BLeSS) to assist full-reference image-quality estimators that originally oversimplify color perception processes. More specifically, the spatiochromatic model is based on spatial frequency, spatial orientation, and surround contrast effects. The assistant similarity method is used to complement image-quality estimators based on phase congruency, gradient magnitude, and spectral residual. The effectiveness of BLeSS is validated using FSIM, FSIMc and SR-SIM methods on LIVE, Multiply Distorted LIVE, and TID 2013 databases. In terms of Spearman correlation, BLeSS enhances the performance of all quality estimators in color-based degradations and the enhancement is at 100% for both feature- and spectral residual-based similarity methods. Moreover, BleSS significantly enhances the performance of SR-SIM and FSIM in the full TID 2013 database.

==> Preprint for ArXiv/tab_bills_results_spearman.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Performance of the BILLS-IQA metrics}
\label{tab_pooling_spatial_all}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
{\bf Distortion Type}                & {\bf Database}                  & {\bf PSNR}   & {\bf SSIM} &{\bf PSNRHA} & {\bf FSIMc} &{\bf PerSIM}  &{\bf SR-SIM}  \\ \hline
\multirow{4}{*}{{\bf Compression}}   & {\bf Jp2k {[}LIVE{]}}           &&&&&&          \\ \cline{2-8} 
                                     & {\bf Jpeg {[}LIVE{]}}           &&&&&&          \\ \cline{2-8} 
                                     & {\bf Compression {[}TID13{]}}   &&&&&&          \\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &&&&&&         \\ \hline
\multirow{3}{*}{{\bf Noise}}         & {\bf Wn {[}LIVE{]}}             &&&&&&   		\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &&&&&&        	\\ \cline{2-8} 
                                     & {\bf Noise {[}TID13{]}}         &&&&&&          \\ \hline
\multirow{2}{*}{{\bf Communication}} & {\bf FF {[}LIVE{]}}             &&&&&&          \\ \cline{2-8} 
                                     & {\bf Communication {[}TID13{]}} &&&&&&   		\\ \hline
\multirow{4}{*}{{\bf Blur}}          & {\bf GBlur {[}LIVE{]}}          &&&&&&         	\\ \cline{2-8} 
                                     & {\bf Blur {[}TID13{]}}          &&&&&&  		\\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &&&&&&      	\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &&&&&&      	\\ \hline
{\bf Color}                          & {\bf Color {[}TID13{]}}         &&&&&&   		\\ \hline
{\bf Global}                      & {\bf Global {[}TID13{]}}     	   &&&&&&         	\\ \hline
{\bf Local}                          & {\bf Local {[}TID13{]}}         &&&&&&         	\\ \hline
\multirow{3}{*}{{\bf All}}           & {\bf All {[}LIVE{]}}            &&&&&&         	\\ \cline{2-8} 
                                     & {\bf All {[}Multi{]}}           &&&&&&         	\\ \cline{2-8} 
                                     & {\bf All {[}TID13{]}}           &&&&&&        	\\ \hline
\end{tabular}
\end{table*}

==> Preprint for ArXiv/tab_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Performance of the IQA metrics based on Spearman correlation}
\label{tab_results}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{{\bf Distortion Type}}                & \multirow{2}{*}{{\bf Database}}  & \multirow{2}{*}{{\bf SR-SIM}} &{{\bf BLeSS}} & \multirow{2}{*}{{\bf FSIM}} &{{\bf BLeSS}} & \multirow{2}{*}{{\bf FSIMc}} &{{\bf BLeSS}}  \\
& & &\textbf{SR-SIM} & &\textbf{FSIM} & &\textbf{FSIMc} \\ \hline 

\multirow{4}{*}{{\bf Compression}}   & {\bf Jp2k {[}LIVE{]}}           &0.972&0.953 &0.981&0.982&0.982&0.980          \\ \cline{2-8} 
                                     & {\bf Jpeg {[}LIVE{]}}           &0.954&0.934 &0.962&0.961  &0.962&0.959       \\ \cline{2-8} 
                                     & {\bf Compression {[}TID13{]}}   &0.967&        0.941 &0.960&0.959&0.961&0.960 \\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.862&         0.866 &0.854&0.857&0.855&0.854 \\ \hline
\multirow{3}{*}{{\bf Noise}}         & {\bf Wn {[}LIVE{]}}             &0.986&0.983   		&0.979&0.980&0.983&0.984\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.863&0.860         	&0.864&0.863&0.869&0.865\\ \cline{2-8} 
                                     & {\bf Noise {[}TID13{]}}         &0.900&0.894          &0.887&0.887&0.897&0.898\\ \hline
\multirow{2}{*}{{\bf Communication}} & {\bf FF {[}LIVE{]}}             &0.966&0.934          &0.970&0.964&0.971&0.964\\ \cline{2-8} 
                                     & {\bf Communication {[}TID13{]}} &0.907&0.897   		&0.895&0.895&0.899&0.912\\ \hline
\multirow{4}{*}{{\bf Blur}}          & {\bf GBlur {[}LIVE{]}}          &0.978&        0.966 	&0.983&0.983&0.983&0.983\\ \cline{2-8} 
                                     & {\bf Blur {[}TID13{]}}          &0.950&0.947  		&0.947&0.948&0.946&0.949\\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.862&0.866        	&0.854&0.857&0.855&0.854\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.863&0.860      	&0.864&0.863&0.869&0.865\\ \hline
{\bf Color}                          & {\bf Color {[}TID13{]}}         &0.243&0.677   		&0.240&0.521&0.629&0.700\\ \hline
{\bf Global}                      & {\bf Global {[}TID13{]}}     	   &0.391&0.399         	&0.441&0.446&0.439&0.441\\ \hline
{\bf Local}                          & {\bf Local {[}TID13{]}}         &0.810&0.817         	&0.702&0.711&0.705&0.722\\ \hline
\multirow{3}{*}{{\bf All}}           & {\bf All {[}LIVE{]}}            &0.955&0.942         	&0.961&0.961&0.959&0.958\\ \cline{2-8} 
                                     & {\bf All {[}Multi{]}}           &0.866&0.866         	&0.863&0.864&0.866&0.864\\ \cline{2-8} 
                                     & {\bf All {[}TID13{]}}           &0.807&0.840        	&0.801&0.828&0.851&0.861\\ \hline
\end{tabular}
\end{table*}

==> Preprint for ArXiv/tab_results_spearman.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Performance of the IQA metrics based on Spearman correlation}
\label{tab_pooling_spatial_all}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
{\bf Distortion Type}                & {\bf Database}                  & {\bf PSNR}   & {\bf SSIM} &{\bf PSNRHA} & {\bf FSIMc} &{\bf PerSIM}  &{\bf SR-SIM}  \\ \hline
\multirow{4}{*}{{\bf Compression}}   & {\bf Jp2k {[}LIVE{]}}           &0.892&0.980&&0.982&0.977&0.972          \\ \cline{2-8} 
                                     & {\bf Jpeg {[}LIVE{]}}           &0.919&0.961&&0.962&0.958&0.954          \\ \cline{2-8} 
                                     & {\bf Compression {[}TID13{]}}   &0.901&0.935&&0.961&0.964&0.967          \\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.619&0.848&&0.855&0.812&0.862          \\ \hline
\multirow{3}{*}{{\bf Noise}}         & {\bf Wn {[}LIVE{]}}             &0.989&0.982&&0.983&0.991&0.986   		\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.593&0.876&&0.869&0.818&0.863         	\\ \cline{2-8} 
                                     & {\bf Noise {[}TID13{]}}         &0.653&0.847&&0.897&0.924&0.900          \\ \hline
\multirow{2}{*}{{\bf Communication}} & {\bf FF {[}LIVE{]}}             &0.897&0.974&&0.971&0.945&0.966          \\ \cline{2-8} 
                                     & {\bf Communication {[}TID13{]}} &0.875&0.894&&0.899&0.865&0.907   		\\ \hline
\multirow{4}{*}{{\bf Blur}}          & {\bf GBlur {[}LIVE{]}}          &0.862&0.971&&0.983&0.973&0.977         	\\ \cline{2-8} 
                                     & {\bf Blur {[}TID13{]}}          &0.839&0.922&&0.946&0.949&0.950  		\\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.619&0.848&&0.855&0.812&0.862        	\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.593&0.876&&0.869&0.818&0.863      	\\ \hline
{\bf Color}                          & {\bf Color {[}TID13{]}}         &0.828&0.234&&0.629&0.762&0.243   		\\ \hline
{\bf Global}                      & {\bf Global {[}TID13{]}}     	   &0.125&0.499&&0.439&0.408&0.391         	\\ \hline
{\bf Local}                          & {\bf Local {[}TID13{]}}         &0.137&0.288&&0.705&0.470&0.810         	\\ \hline
\multirow{3}{*}{{\bf All}}           & {\bf All {[}LIVE{]}}            &0.872&0.949&&0.959&0.950&0.955         	\\ \cline{2-8} 
                                     & {\bf All {[}Multi{]}}           &0.554&0.860&&0.866&0.818&0.866         	\\ \cline{2-8} 
                                     & {\bf All {[}TID13{]}}           &0.528&0.741&&0.851&0.853&0.807        	\\ \hline
\end{tabular}
\end{table*}

==> Preprint for ArXiv/visual.tex <==
\begin{figure}[htbp!]
\vspace{-2.50mm}

\begin{minipage}[b]{0.45\linewidth}
  \centering
\includegraphics[width=\linewidth, trim= 25mm 85mm 25mm 80mm]{Figs/original.pdf}
  \vspace{-0.03cm}
  \centerline{\footnotesize{(a)Pristine Image}}%\medskip
    \vspace{-0.30cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.45\linewidth}
  \centering
\includegraphics[width=\linewidth, trim= 25mm 85mm 25mm 80mm]{Figs/distorted.pdf}
  \vspace{-0.03cm}
  \centerline{\footnotesize{(b) Distorted Image }}%\medskip
    \vspace{-0.30cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.45\linewidth}
  \centering
\includegraphics[width=\linewidth, trim= 25mm 85mm 25mm 70mm]{Figs/bills.pdf}
  \vspace{-0.03 cm}
  \centerline{\footnotesize{(c)  BLeSS Map   } }%\medskip
      \vspace{-0.30cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.45\linewidth}
  \centering
\includegraphics[width=\linewidth, trim= 25mm 85mm 25mm 70mm]{Figs/fsim.pdf}
  \vspace{0.03 cm}
  \centerline{\footnotesize{(d) FSIM Map }}%\medskip
      \vspace{-0.30cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.45\linewidth}
  \centering
\includegraphics[width=\linewidth, trim= 25mm 85mm 25mm 70mm]{Figs/fsimc.pdf}
  \vspace{0.03 cm}
  \centerline{\footnotesize{(e)  FSIMc Map  } }%\medskip
      \vspace{-0.30cm}
\end{minipage}
  \vspace{0.20cm}
\hfill
\begin{minipage}[b]{0.45\linewidth}
  \centering
\includegraphics[width=\linewidth, trim= 25mm 85mm 25mm 70mm]{Figs/srsim.pdf}
  \vspace{0.03 cm}
  \centerline{\footnotesize{(f) SR-SIM Map}}%\medskip
      \vspace{-0.30cm}
\end{minipage}
\vspace{-4.0mm}

\caption{Pristine and distorted images with corresponding quality maps.}\vspace{-.5cm}
\label{fig:visual}
\vspace{-2.0mm}
\end{figure}




==> tab_bills_results_spearman.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Performance of the BILLS-IQA metrics}
\label{tab_pooling_spatial_all}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
{\bf Distortion Type}                & {\bf Database}                  & {\bf PSNR}   & {\bf SSIM} &{\bf PSNRHA} & {\bf FSIMc} &{\bf PerSIM}  &{\bf SR-SIM}  \\ \hline
\multirow{4}{*}{{\bf Compression}}   & {\bf Jp2k {[}LIVE{]}}           &&&&&&          \\ \cline{2-8} 
                                     & {\bf Jpeg {[}LIVE{]}}           &&&&&&          \\ \cline{2-8} 
                                     & {\bf Compression {[}TID13{]}}   &&&&&&          \\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &&&&&&         \\ \hline
\multirow{3}{*}{{\bf Noise}}         & {\bf Wn {[}LIVE{]}}             &&&&&&   		\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &&&&&&        	\\ \cline{2-8} 
                                     & {\bf Noise {[}TID13{]}}         &&&&&&          \\ \hline
\multirow{2}{*}{{\bf Communication}} & {\bf FF {[}LIVE{]}}             &&&&&&          \\ \cline{2-8} 
                                     & {\bf Communication {[}TID13{]}} &&&&&&   		\\ \hline
\multirow{4}{*}{{\bf Blur}}          & {\bf GBlur {[}LIVE{]}}          &&&&&&         	\\ \cline{2-8} 
                                     & {\bf Blur {[}TID13{]}}          &&&&&&  		\\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &&&&&&      	\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &&&&&&      	\\ \hline
{\bf Color}                          & {\bf Color {[}TID13{]}}         &&&&&&   		\\ \hline
{\bf Global}                      & {\bf Global {[}TID13{]}}     	   &&&&&&         	\\ \hline
{\bf Local}                          & {\bf Local {[}TID13{]}}         &&&&&&         	\\ \hline
\multirow{3}{*}{{\bf All}}           & {\bf All {[}LIVE{]}}            &&&&&&         	\\ \cline{2-8} 
                                     & {\bf All {[}Multi{]}}           &&&&&&         	\\ \cline{2-8} 
                                     & {\bf All {[}TID13{]}}           &&&&&&        	\\ \hline
\end{tabular}
\end{table*}

==> tab_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Performance of the IQA metrics based on Spearman correlation}
\label{tab_results}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{{\bf Distortion Type}}                & \multirow{2}{*}{{\bf Database}}  & \multirow{2}{*}{{\bf SR-SIM}} &{{\bf BLeSS}} & \multirow{2}{*}{{\bf FSIM}} &{{\bf BLeSS}} & \multirow{2}{*}{{\bf FSIMc}} &{{\bf BLeSS}}  \\
& & &\textbf{SR-SIM} & &\textbf{FSIM} & &\textbf{FSIMc} \\ \hline 

\multirow{4}{*}{{\bf Compression}}   & {\bf Jp2k {[}LIVE{]}}           &0.972&0.953 &0.981&0.982&0.982&0.980          \\ \cline{2-8} 
                                     & {\bf Jpeg {[}LIVE{]}}           &0.954&0.934 &0.962&0.961  &0.962&0.959       \\ \cline{2-8} 
                                     & {\bf Compression {[}TID13{]}}   &0.967&        0.941 &0.960&0.959&0.961&0.960 \\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.862&         0.866 &0.854&0.857&0.855&0.854 \\ \hline
\multirow{3}{*}{{\bf Noise}}         & {\bf Wn {[}LIVE{]}}             &0.986&0.983   		&0.979&0.980&0.983&0.984\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.863&0.860         	&0.864&0.863&0.869&0.865\\ \cline{2-8} 
                                     & {\bf Noise {[}TID13{]}}         &0.900&0.894          &0.887&0.887&0.897&0.898\\ \hline
\multirow{2}{*}{{\bf Communication}} & {\bf FF {[}LIVE{]}}             &0.966&0.934          &0.970&0.964&0.971&0.964\\ \cline{2-8} 
                                     & {\bf Communication {[}TID13{]}} &0.907&0.897   		&0.895&0.895&0.899&0.912\\ \hline
\multirow{4}{*}{{\bf Blur}}          & {\bf GBlur {[}LIVE{]}}          &0.978&        0.966 	&0.983&0.983&0.983&0.983\\ \cline{2-8} 
                                     & {\bf Blur {[}TID13{]}}          &0.950&0.947  		&0.947&0.948&0.946&0.949\\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.862&0.866        	&0.854&0.857&0.855&0.854\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.863&0.860      	&0.864&0.863&0.869&0.865\\ \hline
{\bf Color}                          & {\bf Color {[}TID13{]}}         &0.243&0.677   		&0.240&0.521&0.629&0.700\\ \hline
{\bf Global}                      & {\bf Global {[}TID13{]}}     	   &0.391&0.399         	&0.441&0.446&0.439&0.441\\ \hline
{\bf Local}                          & {\bf Local {[}TID13{]}}         &0.810&0.817         	&0.702&0.711&0.705&0.722\\ \hline
\multirow{3}{*}{{\bf All}}           & {\bf All {[}LIVE{]}}            &0.955&0.942         	&0.961&0.961&0.959&0.958\\ \cline{2-8} 
                                     & {\bf All {[}Multi{]}}           &0.866&0.866         	&0.863&0.864&0.866&0.864\\ \cline{2-8} 
                                     & {\bf All {[}TID13{]}}           &0.807&0.840        	&0.801&0.828&0.851&0.861\\ \hline
\end{tabular}
\end{table*}

==> tab_results_spearman.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Performance of the IQA metrics based on Spearman correlation}
\label{tab_pooling_spatial_all}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
{\bf Distortion Type}                & {\bf Database}                  & {\bf PSNR}   & {\bf SSIM} &{\bf PSNRHA} & {\bf FSIMc} &{\bf PerSIM}  &{\bf SR-SIM}  \\ \hline
\multirow{4}{*}{{\bf Compression}}   & {\bf Jp2k {[}LIVE{]}}           &0.892&0.980&&0.982&0.977&0.972          \\ \cline{2-8} 
                                     & {\bf Jpeg {[}LIVE{]}}           &0.919&0.961&&0.962&0.958&0.954          \\ \cline{2-8} 
                                     & {\bf Compression {[}TID13{]}}   &0.901&0.935&&0.961&0.964&0.967          \\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.619&0.848&&0.855&0.812&0.862          \\ \hline
\multirow{3}{*}{{\bf Noise}}         & {\bf Wn {[}LIVE{]}}             &0.989&0.982&&0.983&0.991&0.986   		\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.593&0.876&&0.869&0.818&0.863         	\\ \cline{2-8} 
                                     & {\bf Noise {[}TID13{]}}         &0.653&0.847&&0.897&0.924&0.900          \\ \hline
\multirow{2}{*}{{\bf Communication}} & {\bf FF {[}LIVE{]}}             &0.897&0.974&&0.971&0.945&0.966          \\ \cline{2-8} 
                                     & {\bf Communication {[}TID13{]}} &0.875&0.894&&0.899&0.865&0.907   		\\ \hline
\multirow{4}{*}{{\bf Blur}}          & {\bf GBlur {[}LIVE{]}}          &0.862&0.971&&0.983&0.973&0.977         	\\ \cline{2-8} 
                                     & {\bf Blur {[}TID13{]}}          &0.839&0.922&&0.946&0.949&0.950  		\\ \cline{2-8} 
                                     & {\bf Blur-Jpeg {[}MULTI{]}}     &0.619&0.848&&0.855&0.812&0.862        	\\ \cline{2-8} 
                                     & {\bf Blur-Noise {[}MULTI{]}}    &0.593&0.876&&0.869&0.818&0.863      	\\ \hline
{\bf Color}                          & {\bf Color {[}TID13{]}}         &0.828&0.234&&0.629&0.762&0.243   		\\ \hline
{\bf Global}                      & {\bf Global {[}TID13{]}}     	   &0.125&0.499&&0.439&0.408&0.391         	\\ \hline
{\bf Local}                          & {\bf Local {[}TID13{]}}         &0.137&0.288&&0.705&0.470&0.810         	\\ \hline
\multirow{3}{*}{{\bf All}}           & {\bf All {[}LIVE{]}}            &0.872&0.949&&0.959&0.950&0.955         	\\ \cline{2-8} 
                                     & {\bf All {[}Multi{]}}           &0.554&0.860&&0.866&0.818&0.866         	\\ \cline{2-8} 
                                     & {\bf All {[}TID13{]}}           &0.528&0.741&&0.851&0.853&0.807        	\\ \hline
\end{tabular}
\end{table*}
